Applications of Deep Learning in Fish Habitat Monitoring: A Tutorial and Survey

Marine ecosystems and their fish habitats are becoming increasingly important due to their integral role in providing a valuable food source and conservation outcomes. Due to their remote and difficult to access nature, marine environments and fish habitats are often monitored using underwater cameras. These cameras generate a massive volume of digital data, which cannot be efficiently analysed by current manual processing methods, which involve a human observer. DL is a cutting-edge AI technology that has demonstrated unprecedented performance in analysing visual data. Despite its application to a myriad of domains, its use in underwater fish habitat monitoring remains under explored. In this paper, we provide a tutorial that covers the key concepts of DL, which help the reader grasp a high-level understanding of how DL works. The tutorial also explains a step-by-step procedure on how DL algorithms should be developed for challenging applications such as underwater fish monitoring. In addition, we provide a comprehensive survey of key deep learning techniques for fish habitat monitoring including classification, counting, localization, and segmentation. Furthermore, we survey publicly available underwater fish datasets, and compare various DL techniques in the underwater fish monitoring domains. We also discuss some challenges and opportunities in the emerging field of deep learning for fish habitat processing. This paper is written to serve as a tutorial for marine scientists who would like to grasp a high-level understanding of DL, develop it for their applications by following our step-by-step tutorial, and see how it is evolving to facilitate their research efforts. At the same time, it is suitable for computer scientists who would like to survey state-of-the-art DL-based methodologies for fish habitat monitoring.

==> table_cls.tex <==
% \usepackage{array}
% \usepackage{graphicx}
% \usepackage{colortbl}


\begin{table*}
\begin{sideways}
\begin{minipage}{\textheight}

\centering
\caption{Classification}
\label{table:cls}
\arrayrulecolor[rgb]{0.647,0.647,0.647}
\resizebox{\linewidth}{!}{%
\begin{tabular}{>{\hspace{0pt}}p{0.18\linewidth}>{\hspace{0pt}}p{0.05\linewidth}>{\hspace{0pt}}p{0.044\linewidth}>{\hspace{0pt}}p{0.16\linewidth}>{\hspace{0pt}}p{0.16\linewidth}>{\hspace{0pt}}p{0.100\linewidth}>{\hspace{0pt}}p{0.048\linewidth}>{\hspace{0pt}}p{0.069\linewidth}>{\hspace{0pt}}p{0.186\linewidth}}
\arrayrulecolor{black}\hline
\multicolumn{1}{>{\centering\hspace{0pt}}m{0.18\linewidth}}{\textbf{Article }} & \multicolumn{1}{>{\centering\hspace{0pt}}m{0.05\linewidth}}{\textbf{ DL Model Used }} & \multicolumn{1}{>{\centering\hspace{0pt}}m{0.044\linewidth}}{\textbf{ Framework }} & \multicolumn{1}{>{\centering\hspace{0pt}}m{0.16\linewidth}}{\textbf{ Data }} & \multicolumn{1}{>{\centering\hspace{0pt}}m{0.16\linewidth}}{\textbf{ ~ annotation  Pre-processing  augmentation }} & \multicolumn{1}{>{\centering\hspace{0pt}}m{0.100\linewidth}}{\textbf{ Classes and Labels }} & \multicolumn{1}{>{\centering\hspace{0pt}}m{0.048\linewidth}}{\textbf{ Performance Metric }} & \multicolumn{1}{>{\centering\hspace{0pt}}m{0.069\linewidth}}{\textbf{ Value of Metric Used }} & \multicolumn{1}{>{\centering\arraybackslash\hspace{0pt}}m{0.186\linewidth}}{\textbf{ Comparisons with other methods }} \\
\arrayrulecolor[rgb]{0.647,0.647,0.647}\hline


  
   \rowcolor[rgb]{0.929,0.929,0.929}  Recognition Of Fish Categories Using Deep Learning Technique \cite{Varalakshmi2019a}& CNN & Keras- Tensorflow & 560
  Authors-created dataset containing
  ~560 fish images,
  400 train and 160 test. & Image of a single fish and associating a label (i.e.
  species name) & 10 classes :10 different fish species. & CA & 95\% & NA \\
  
    Comparison of Different Deep Structures for Fish Classification \cite{Sarigul2017c} & CNN & Torch & The public QUT fish dataset 
  contains 3960 images of 468 species of fish in different environments. & Image of a single fish and associating a label (i.e. species name) & 468 ~classes: 468 ~Different
  fish species & CA & 46.02\% & NA \\
  
    \rowcolor[rgb]{0.929,0.929,0.929}  Fish species classification in unconstrained underwater
  environments based on deep learning \cite{Salman2016} & CNN & NA & The images are from a public dataset 
  ~Fish4Knowledge (LifeCLEF 2014, LifeCLEF
  2015) & Image of a single fish and associating a label (i.e. species name) & 25 classes :25 different fish species. & CA & 96.75\% & Comparison with conventional machine learning tools as SVM methods 83.94\% \\
 
   DeepFish: Accurate underwater live fish recognition with a deep architecture \cite{Qin2016a} & CNN & Matlab & The images are from a public dataset 
  ~Fish4Knowledge & Image of a single fish and associating a label (i.e. species name) & 23 classes: 23 Different
  fish species & CA & 98.64\% & Comparison with conventional machine learning tools as baseline methods 93.58\% \\
  
   \rowcolor[rgb]{0.929,0.929,0.929} Fish recognition from low-resolution underwater images \cite{Sun2017a} & CNN & NA & 93 videos from LifeCLEF 2015 fish dataset
  ~ & bounding box and species name & 15 classes :15 different fish species. & CA & 76.57\% & Authors used the~~
  traditional~~ gabor~~ features~~
  and~~ dense~~ sift~~
  features with~ 38.28\% ,~~~~ 28.63\% respectively
  dataset as~
  comparison~ methods. \\
  
  Automatic Fish Classification System
  Using Deep Learning \cite{Chen2018c} & CNN & NA & Eight target categories are available in this dataset:
  Albacore tuna, Bigeye tuna, Yellowfin tuna, Mahi Mahi, Opah, Sharks, Other. & Image of a single fish and associating a label (i.e.
  species name) & 8 classes: 8 Different
  fish species. & CE & 0.578
  1.387 & Kaggle leaderboard
  0.578 cross entropy (rank: 17th) on test
  set at stage 1 and 1.387 (rank: 16th) at stage 2. \\
  
   \rowcolor[rgb]{0.929,0.929,0.929}  A realistic fish-habitat dataset to evaluate algorithms
  for underwater visual analysis \cite{Saleh2020}
  ~ & ~ResNet-50 CNN & Pytorch & Authors-created database containing
  ~39,766~ images From ~ 20 habitats from remote coastal
  marine environments of tropical Australia & point-level and semantic segmentation labels & 20 classes: 20 Different
  fish habitat. & CA & 0.99
  ~ & NA \\

   Deep learning for underwater image recognition in small
  sample size situations \cite{Jin2017a} & CNN & Caffe & The images are from a public dataset 
  ~Fish4Knowledge & Image of a single fish and associating a label (i.e.
  species name) & 10 classes: 10 Different
  fish species & CA & 85.08\% & NA \\
 
  \rowcolor[rgb]{0.929,0.929,0.929}  Underwater Fish Species Classification using Convolutional Neural Network and Deep Learning \cite{Rathi_2017} & CNN & NA & \textasciitilde{}27000 images from a public dataset 
  ~Fish4Knowledge & Image of a single fish and associating a label (i.e.
  species name) & 23 classes :23 different fish species. & CA & 96.29\% & NA \\
 
  Underwater Live Fish Recognition
  by Deep Learning \cite{Tamou2018a} & AlexNet ~- CNN & Matlab & \textasciitilde{}27000 images from a public dataset 
  ~Fish4Knowledge & Image of a single fish and associating a label (i.e.
  species name) & 23 classes :23 different fish species. & CA & 99.45\%. & NA \\

  \rowcolor[rgb]{0.929,0.929,0.929}  WildFish++: A Comprehensive Fish Benchmark for Multimedia Research \cite{Zhuang2020} & CNN & NA & Authors created a data set of 54,459 labelled ~~images from various professional websites and
  Google engine. & Image of a single fish and associating a label (i.e.
  species name) & 100 classes :1000 different fish species. & CA & 74.7\% & Comparison with other state-of-the-art approaches \\

 Automatic fish species classification in underwater videos:
exploiting pre-trained deep neural network models to
compensate for limited labelled data \cite{Siddiqui2018a} & CNN & MATLAB & Video clips of the 16 species from Western Australia during 2011–2013., between
  50 and 120 individual 10 second video clips of each of the 16 focal species
  were captured. & Image of a single fish and associating a label (i.e. species name) & 16 classes: 16 Different
  fish species & CA & 89.0\% & Comparing with two existing classification methods; 
  SRC (Hsiao \textit{et al.}\cite{HSIAO201413}) 49.1\%
  CNN (Salman \textit{et al.}\cite{Salman2016}) 53.5\%
  Proposed method of CNN plus SVM  89.0\% \\
  
  
  \rowcolor[rgb]{0.929,0.929,0.929}  Underwater Fish Species Recognition using Deep
  Learning Techniques \cite{Deep2019a} & CNN & Keras- Tensorflow & \textasciitilde{}35000 images from a public dataset 
  ~Fish4Knowledge & Image of a single fish and associating a label (i.e. species name) & 23 classes :23 different fish species. & CA & 98.79\% & NA \\
  
  Automatic Fish Species Classification Using Deep
  Convolutional Neural Networks \cite{Iqbal2021a} & modified AlexNet
  CNN & Tensorflow & The images are from two public datasets 
  QUT fish dataset 
  LifeClef-15 & Image of a single fish and associating a label (i.e.
  species name) & 6 classes: 6 Different
  fish species & CA & 90.48\% & Comparing modified AlexNet
  90.48\% with original AlexNet
  86.65\% \\
  
   \rowcolor[rgb]{0.929,0.929,0.929} Underwater Fish Detection with Weak
  Multi-Domain Supervision \cite{Konovalov2019a} & CNN & Keras- Tensorflow & Authors created a data set of 40000 labelled ~~images from video sequences & Fish/no fish & 1 class & CA & 99.94\% & NA \\
  
  A Deep learning method for accurate and fast identification of coral reef fishes in underwater images \cite{Villon2018a} & GoogLeNet CNN & Caffe & Authors-created database containing 450,000
  Images from 116 over 50 reef sites around the Mayotte
  island
  ~ & annotation consisted in drawing a rectangle bounding box
  around a single fish individual and associating a label (i.e. species name)
  to this individual. & 20 classes: 20 Different
  fish species. & CA & 94.9\% & Comparing accuracy to human experts 
  The rate of correct identification was 94.9\%, greater
  than the rate of correct identification by humans
  (89.3\%). \\

 \rowcolor[rgb]{0.929,0.929,0.929} Underwater-Drone With Panoramic Camera for Automatic Fish Recognition Based on Deep Learning \cite{Meng2018a} & CNN & NA & Authors created a data set of 100 labelled ~~images from Google search
  engine. & Image of a single fish and associating a label (i.e. species name) & 4 classes :4 different fish species. & CA & 87\% & NA \\
  










\hline
\end{tabular}
}
\arrayrulecolor{black}


\end{minipage}
\end{sideways}
\end{table*}
